Symmetry-Aware Predicate Abstraction for Shared-Variable Concurrent Programs (Extended Technical Report)

Predicate abstraction is a key enabling technology for applying finite-state model checkers to programs written in mainstream languages. It has been used very successfully for debugging sequential system-level C code. Although model checking was originally designed for analyzing concurrent systems, there is little evidence of fruitful applications of predicate abstraction to shared-variable concurrent software. The goal of this paper is to close this gap. We have developed a symmetry-aware predicate abstraction strategy: it takes into account the replicated structure of C programs that consist of many threads executing the same procedure, and generates a Boolean program template whose multi-threaded execution soundly overapproximates the concurrent C program. State explosion during model checking parallel instantiations of this template can now be absorbed by exploiting symmetry. We have implemented our method in the SATABS predicate abstraction framework, and demonstrate its superior performance over alternative approaches on a large range of synchronization programs.

==> model-checking.tex <==
% Commands for model checking domain

\newcommand{\Aut}       {\operatorname{\mathit{Aut}}}     % automorphism group
\newcommand{\Auto}      {\operatorname{\mathit{Auto}}}    % automorphism group
\newcommand{\Sym}       {\operatorname{\mathit{Sym}}}     % Symmetry group
\newcommand{\Orbit}     {\mathit{Orbit}}
\newcommand{\bad}       {\mathit{bad}}
\newcommand{\good}      {\mathit{good}}
\newcommand{\init}      {\mathit{init}}
\newcommand{\req}       {\mathit{req}}
\newcommand{\grant}     {\mathit{grant}}
\newcommand{\ready}     {\mathit{ready}}
\newcommand{\exec}      {\mathit{exec}}
\newcommand{\Reached}   {\mathit{Reached}}
\newcommand{\Unexplored}{\mathit{Unexplored}}
\newcommand{\halts}[3][]{#2 \downarrow^{#1} #3}
\newcommand{\sts}       {\vdash}                          % single turnstyle
\newcommand{\dts}       {\models}                         % double turnstyle
\newcommand{\tts}       {\,\operatorname{\mid\!\equiv}\,} % triple turnstyle
\newcommand{\sat}       {\models}                         % "satisfies"
\newcommand{\AP}        {\mathit{AP}}                     % set of atomic propositions AP
\newcommand{\pc}        {\mathit{pc}}
\newcommand{\bisim}     {\approx}
\newcommand{\nondet}    {\star}

% For synchronization skeletons, etc
\newcommand{\edge}[3]{{#1} \stackrel{{#2}}{    \rightarrow} {#3}} % short argument #2
\newcommand{\Edge}[3]{{#1} \stackrel{{#2}}{\longrightarrow} {#3}} % long  argument #2
\newcommand{\self}{\mathit{self}}
\newcommand{\odeg}{\deg_{\operatorname{out}}}                     % out-degree of a vertex
\newcommand{\ideg}{\deg_{\operatorname{in}}}                      % in- degree of a vertex


% Tools

\newcommand{\bebop}  {\tool{Bebop}}
\newcommand{\boom}   {\tool{Boom}}
\newcommand{\bboom}  {\tool{B-Boom}}
\newcommand{\cbmc}   {\tool{Cbmc}}
\newcommand{\getafix}{\tool{GetAFix}}
\newcommand{\moped}  {\tool{Moped}}
\newcommand{\murphi} {\tool{Mur$\varphi$}}
\newcommand{\nusmv}  {\tool{NuSMV}}
\newcommand{\promela}{\tool{ProMeLa}}
\newcommand{\satabs} {\tool{SatAbs}}
\newcommand{\slam}   {\tool{Slam}}
\newcommand{\spin}   {\tool{Spin}}
\newcommand{\sviss}  {\tool{Sviss}}
\newcommand{\boppo}   {\tool{Boppo}}


\newcommand{\Rep}{\mathit{Rep}}

\newcommand{\Mbar}   {\bar{M}}                               % quotient structure
\newcommand{\Sbar}   {\bar{S}}
\newcommand{\Rbar}   {\bar{R}}
\newcommand{\Lbar}   {\bar{L}}
\newcommand{\sbar}   {\bar{s}}
\newcommand{\tbar}   {\bar{t}}
\newcommand{\APbar}  {\bar{\AP}}
\newcommand{\badbar} {\overline{\mathit{bad}}}
\newcommand{\goodbar}{\overline{\mathit{good}}}
\newcommand{\initbar}{\overline{\mathit{init}}}

\newcommand{\Mhat}{\widehat{M}}                                   % annotated quotient structure; generic structure
\newcommand{\Shat}{\widehat{S}}
\newcommand{\Rhat}{\widehat{R}}
\newcommand{\Lhat}{\widehat{L}}
\newcommand{\Phat}{\widehat{\P}}
\newcommand{\shat}{\hat{s}}
\newcommand{\that}{\hat{t}}

\newcommand{\modality}[1]{\operatorname{\mathsf{#1}}}             % Temporal Logic operators

% LTL temporal operators
\newcommand{\X}  {\modality{X}}
\newcommand{\F}  {\modality{F}}
\newcommand{\G}  {\modality{G}}
\newcommand{\U}  {\modality{U}}
\newcommand{\GF} {\modality{GF}}
\newcommand{\FG} {\modality{FG}}

% Path quantifiers
\newcommand{\E}  {\modality{E}}
\newcommand{\A}  {\modality{A}}

% Future-time CTL modalities
\newcommand{\EX} {\modality{EX}}
\newcommand{\AX} {\modality{AX}}
\newcommand{\EF} {\modality{EF}}
\newcommand{\AF} {\modality{AF}}
\newcommand{\EG} {\modality{EG}}
\newcommand{\AG} {\modality{AG}}
\newcommand{\EU} {\modality{EU}}
\newcommand{\AU} {\modality{AU}}

% Past-time CTL modalities
\newcommand{\EY} {\modality{EY}}
\newcommand{\AY} {\modality{AY}}
\newcommand{\EP} {\modality{EP}}

\newcommand{\INV}{\modality{INV}}

\newcommand{\image}{\modality{Im}}
\newcommand{\Image}{\modality{Image}}
\newcommand{\PreIm}{\modality{PreIm}}

% Misc
\newcommand{\mucalc}{$\mu$-calculus\xspace}


==> theorems.tex <==
% Theorem-like environments. All theorems, lemmata, etc. are numbered
% like equations, such that in effect there is only one counter to be
% referred to.

\newtheorem{DEF}     {Definition}%[section] % this may cause problems...
\newtheorem{THE}[DEF]{Theorem}
\newtheorem{LEM}[DEF]{Lemma}
\newtheorem{PRO}[DEF]{Property}
\newtheorem{CLA}[DEF]{Claim}
\newtheorem{OBS}[DEF]{Observation}
\newtheorem{REQ}[DEF]{Requirement}
\newtheorem{COR}[DEF]{Corollary}
\newtheorem{CON}[DEF]{Conjecture}

% Proofs and results

% \proof clashes with llncs,fac,...
\newcommand{\Proof}{\textbf{Proof}\xspace}              % introducing a proof
\newcommand{\explain}[1]{\tab \angles{\mbox{#1}}}       % explanations in proofs in Dijkstra notation
\newcommand{\eop}[1][3mm]{\eopBox \vspace{#1}}          % end of proof (box), followed by new paragraph. Use:
                                                        % \begin{THE}
                                                        %   Bla.
                                                        % \end{THE}
                                                        % \Proof: Bla.
                                                        % This completes the proof.\eop
                                                        %     <empty line in the text>
                                                        % Next we ...

\newcommand{\eopBox}{~\hfill$\Box$}                     % box at end of proof. Use only where new paragraph
                                                        % is illegal or unwanted, as before another "section", etc. command

% About the \eop family: ~ enforces blank before \Box, even if space is tight.
% No space before \eop in the text, otherwise the line might be broken right before \eop!
% To avoid indentation in paragraph after proof, use
% "... completes the proof.\eop

% \noindent
% Next, ..."

% If you have more space, use an indented proof environment:
\newenvironment{PROOF}[1][\Proof:]{\begin{description} \item[#1]\mbox{}}{\end{description}}
% Use:
% \begin{THE}
%   BLA.
% \end{THE}
% \begin{PROOF}
%   % newline here if desired
%   Bla Proof.\eop
% \end{PROOF}
%   <empty line optional, has no vertical space effect, but starts new paragraph and thus indents.>
% Next we ...


%When repeating theorems, say in order to export its proof to an appendix,
%you want to reuse the original counter value. Do this as follows:

%Main text:
%\newcounterset{uniqueLabel}{\theDEF}
%\begin{THE}
%  \label{theorem: uniqueLabel}
%  Bla
%\end{THE}

%Appendix:
%\setcounter{DEF}{\value{uniqueLabel}}
%\begin{THE}
%  Bla
%\end{THE}

%Do not repeat the \label command in the second mention of the theorem.

